Safety Representations for Safer Policy Learning

Reinforcement learning algorithms typically necessitate extensive exploration of the state space to find optimal policies. However, in safety-critical applications, the risks associated with such exploration can lead to catastrophic consequences. Existing safe exploration methods attempt to mitigate this by imposing constraints, which often result in overly conservative behaviours and inefficient learning. Heavy penalties for early constraint violations can trap agents in local optima, deterring exploration of risky yet high-reward regions of the state space. To address this, we introduce a method that explicitly learns state-conditioned safety representations. By augmenting the state features with these safety representations, our approach naturally encourages safer exploration without being excessively cautious, resulting in more efficient and safer policy learning in safety-critical scenarios. Empirical evaluations across diverse environments show that our method significantly improves task performance while reducing constraint violations during training, underscoring its effectiveness in balancing exploration with safety.

==> sections/background.tex <==
\section{Preliminaries}

RIPL may be applied to both constrained and unconstrained MDPs. Here, we review the notation and central concepts for these decision-making models.

\subsection{Markov Decision Processes} 

Markov decision processes (MDPs) are defined as a tuple $\langle S, A, T, R, d, \gamma \rangle$, where $S$ is a set of states; $A$ is a set of actions; $R: S \times A \times S \rightarrow \mathbb{R}$ is the reward function indicating the immediate reward for executing action $a$ in state $s$ and resulting in state $s'$; $T: S \times A \times S \rightarrow [0, 1]$ is the forward dynamics model indicating the probability of achieving state $s'$ after executing action $a$ in state $s$; $d: S \rightarrow [0, 1]$ represents the probability of starting in a state $s \in S$; and $\gamma \in [0, 1)$ is a discount factor.

A solution to an MDP is a policy $\pi: S \rightarrow A$ that prescribes an action $\pi(s)$ for each state $s \in S$. Policies may be stochastic, written as $\pi(a|s)$, indicating the probability of choosing action $a$ when in state $s$. The optimal solution to an MDP is an optimal policy $\pi^*$ that maximizes the expected cumulative discounted reward, $J(\pi)$:
\begin{equation}
    J(\pi) = \mathbb{E}_{s_0 \sim d(s)} \Big [ \mathbb{E}_{\tau_{s_0} ^{\pi}} \Big [ \sum_{t=0}^{\infty} \gamma^t R(s_t, a_t, s_{t+1)} \Big ] \Big ].
\end{equation}

Here, $\tau_{s_0} ^{\pi}$ is a sequence of states generated by executing policy $\pi$ starting from state $s_0$. Executing a policy $\pi$ induces a value function $V^{\pi}: S \rightarrow \mathbb{R}$ indicating the expected cumulative discounted reward that an agent would experience if it executed policy $\pi$ beginning in state $s$. The optimal policy $\pi^*$ induces the maximum value function for each state $V^*$.

\subsection{Constrained Markov Decision Processes} 

Constrained MDPs (CMDPs) are defined as a tuple $\langle S, A, T, R, d, \gamma, \mathcal{C}, \beta \rangle$, where $S$, $A$, $T$, $R$, $d$, and $\gamma$ retain their MDP definitions. $\mathcal{C}: S \rightarrow \mathbb{R}^+$ is a cost function, mapping each state to a real-valued, non-negative cost. $\beta$ is budget, or a maximum, cumulative cost that is acceptable in expectation. The optimal solution to a CMDP is a policy $\pi^*$ that, again, maximizes the expected cumulative discounted reward, but also accumulates expected discounted cost less than   $\beta$:
\begin{equation}
    \begin{array}{cc}
        J(\pi) =&\hspace{-2mm}\mathbb{E}_{s_0 \sim d(s)} \Big [ \mathbb{E}_{\tau_{s_0} ^{\pi}} \Big [ \displaystyle \sum_{t=0}^{\infty} \gamma^t R(s_t, a_t, s_{t+1)} \Big ] \Big ]. \\
        \text{s.t.} & \mathbb{E}_{s_0 \sim d(s)} \Big [ \mathbb{E}_{\tau_{s_0} ^{\pi}} \Big [ \displaystyle \sum_{t=0}^{\infty} \gamma^t \mathcal{C}(s_t) \Big ] \Big ] \leq \beta. \\
    \end{array}
\end{equation}

Intuitively, we can view the constraints imposed by $\mathcal{C}$ and $\beta$ as reducing the set of possible policies from all policies $\Pi$ to those satisfying the constraints $\Pi_{\mathcal{C}} \subseteq \Pi$. While $\pi^*$ is deterministic for MDPs, it is generally stochastic in CMDPs as this allows agents to fully exploit $\beta$ in expectation. \todo{Samer can find a reference for this?... also move to footnote}

In deep reinforcement learning (DRL), due to approximation errors, it is typically impossible to guarantee that the agent will never execute a policy $\pi \notin \Pi_{\mathcal{C}}$ during training. Therefore, in the absence of any prior information, the agent will likely violate the constraints during exploration. Given this, we often care about both the cumulative cost incurred during training as well as the expected cost of the final policy.

\subsection{``Safety'', ``Risk'', and Important Assumptions}

The reinforcement learning community has adopted several terms to describe the behaviour of agents exhibiting some sense of self-preservation or some concept of the broader consequences of their actions, ``risk-aware'' and ``safe'' among the most prominent\footnote{This is separate from notions of ``ethical'' or ``fair'' decision making, though the consensus is still evolving~\citep{nashed2023fairness}.}. Even among RL researchers these terms often index subtly different meanings or reasoning mechanisms that may differ from their use in other areas of sequential decision-making and may depart entirely from their non-technical denotation. In this paper we do not attempt to unify, classify, or intentionally reify any particular terms adopted from colloquial speech, though the general concept of ``risk'' comes closest to the intuition used to design RIPL. In the remainder of the paper, we will collectively refer to states we wish to avoid (terminal states in the unconstrained case, and cost-inducing states in the constrained case) as ``unsafe'' states. A state of course may have high risk in that it is near an unsafe state, but may not be unsafe itself.

Despite the state of terminology, RL researchers have remained fairly consistent in the assumptions they make about their operating environments. We follow two of the most common in the literature~\citep{learning_to_be_safe,ldm,csc}: (1) \emph{Identifiability}: Unsafe states are identifiable as such, either via episode termination or immediate accumulation of cost or reward. (2) \emph{Binary Safety}: The categorization of a state as safe or unsafe is binary; varying degrees of safety are not considered and we use strictly $\mathcal{C}: \mathcal{S} \rightarrow \{0, 1\}$.

Though they do exclude some decision-making models, these assumptions allow a large, informal class of MDPs. For example, any CMDP for which there is some subset of states $S_{unsafe} \subset S$ which induce a non-zero, constant cost. Or, any MDP with absorbing states or sink states $S_{unsafe} \subset S$ that, when the agent enters, terminate the episode prematurely and may or may not produce negative reward. Although most of the example domains in safety gym \citep{safety-gym} and other popular RL environments represent safety as a physical property, the concept of unsafe states, and thus the RIPL framework, may be applied to any MDP following the above assumptions, whether or not the label of ``unsafe'' is accurate in a colloquial sense. \todo{add robotics examples (non-ergodic state, reset state, etc.)}


==> sections/intro.tex <==
\section{Introduction}


% \begin{itemize}
%     \item In nature, organisms have a model of the riskiness of states learned through play, self play, social, innate, whatever. This helps them learn new envs, operate safely, learn more efficiently, etc.
%     \item We devise a machinery to endow RL agents with such a risk model. Indeed, we <description of the machinery>
%     \item We then review the impact of this additional system on commonly-studied aspects of RL artificial life. For instance: safety during training, safety after training, efficiency of training, transferrability to new tasks.
% \end{itemize}

% \begin{itemize}
%     \item SN todo:
%     \item P6: Summary of results... possibly combine with above.
% \end{itemize}



%details about the training and such can be moved to the later section. I think what Liam said about Implicit bias and generalization those two points can be emphasised

Reinforcement Learning (RL) environments often incorporate the notion of failure, where certain events are deemed undesirable during both training and deployment. To manage these failures, RL frameworks 
employ negative rewards or enforce constraints that penalize the agent for unsafe actions. The primary challenge lies in training an agent that can navigate an uncertain and potentially hazardous environment while balancing the risk of failure against the reward for task completion. During the exploration phase, the agent must contend with the inherent epistemic uncertainty of the environment, making it particularly difficult to avoid failures that are not yet fully understood. This challenge is further compounded in scenarios where safety and task objectives are misaligned, such as in the Safety Gym environment or autonomous driving, where optimizing for speed may compromise safety measures like avoiding collisions.

In environments where safety and task objectives are more closely aligned, such as robotic manipulation tasks, the learning process presents a different set of challenges. Here, the agent may quickly learn that certain actions are risky, leading to overly conservative behaviours that inhibit further exploration. This premature convergence to a risk-averse policy not only results in sample inefficiency but also hinders the agent's ability to learn more complex, state-conditioned representations that are crucial for achieving the task. Consequently, the agent’s exploration is curtailed, resulting in a learning process that is both inefficient and unsafe. This issue underscores the broader difficulty of deploying RL algorithms in real-world settings, where the need for both efficient learning and adherence to safety constraints is paramount.





We propose to ease the learning of state-conditioned risk by introducing an implicit bias. An additional low-dimensional state risk representation is added to the agent's observations. This representation allows for faster learning of state-conditioned risk in the critic and policy, allowing the agent to reach higher performance faster and avoid unsafe states during training. This representation is learned explicitly using the experience gathered during training as a quantile distribution over distance to failure.  We show that this leads to significantly higher performance in both cases of safety/task relationships. This uses the insight that risk is state-conditioned. This leads to the ability to transfer across tasks in the same environment.   


%%% Sept 2nd 2024
%Reinforcement learning (RL) has shown promise as a paradigm for solving sequential decision-making problems in a variety of domains, including games~\citep{shao2019survey}, recommender systems~\citep{afsar2022reinforcement}, infrastructure control~\citep{arwa2020reinforcement,chen2022reinforcement,degrave2022magnetic}, and robotics~\citep{zhang2021reinforcement,singh2022reinforcement}. Nonetheless, there are several key challenges that prevent more widespread adoption of RL-based systems, of which we highlight three. (1) \emph{Sample efficiency:} RL algorithms require more data to train than is feasible in many scenarios, especially in robotics. (2) \emph{Transferability / Generalization:} It is often difficult to extract task-agnostic information from a policy trained to complete a particular task in order to learn a new task in the same environment. (3) \emph{Safety during exploration:} While the process of exploration is inherently risky and there is some amount of risk that is irreducible, state-of-the-art ``safe'' RL algorithms still make more mistakes than many applications can afford\footnote{In many applications, the risks of taking the wrong action are relatively benign: a user is served an inaccurate ad or a movie recommendation they have no interest in, or the agent dies in a video game and must start the level over again. However, action selection for agents operating in the physical world often presents significant risk: robotic systems, such as autonomous vehicles, can cause severe injury to themselves or their human counterparts, power-grid management systems can disrupt peoples' access to reliable electricity, and healthcare agents could dramatically change patients' conditions. Although such systems often have access to simulators in which they may conduct a large amount of low-risk training, the so-called sim-to-real gap will likely remain a challenge for many applications~\citep{salvato2021crossing}.}. 

%One aspect of learning hypothesized to be important is disentangling task- and environment-specific information~\citep {mao2018universal,kim2019curiosity,zhou2019environment}. This is built largely on the intuition that, in many environments, states possess action-independent properties that are correlated with their induced value (or cost) under many policies. For example, driving in the opposite lane on a two-lane road is more risk-prone regardless of the policy the agent follows. In fact, the concept of state-dependent risk may guide human skill acquisition, in part through an awareness that certain behaviours or elements in our environment pose inherent risks \citep{simpson1996neither}, and is thought to have broad utility in learning complex, dangerous tasks \citep{keating2008adolescent}. Regardless of the task at hand, we instinctively avoid certain states with the \emph{potential} for harm, enabling us to navigate novel scenarios judiciously when learning \citep{crawford2002learning}.


% Motivated by these insights from human learning, we introduce a novel approach to represent the underlying structure of hazards in the environment via the acquisition of an independent \emph{risk model} which is simultaneously (or subsequently) used to condition the RL agent.



%Motivated by these insights from human learning, we propose a novel approach to learning a representation that models the risk associated with a state, introducing an implicit bias into the policy learning process. By embedding risk information directly into the state representation, we enable risk-aware learning, allowing the agent to make more informed and cautious decisions in high-risk situations. This approach is particularly advantageous in high-dimensional state spaces, where effective risk modelling becomes increasingly critical. Assuming that the cost function remains consistent across tasks—meaning the inherent characteristics of objects or states do not change—we propose a policy-agnostic risk modelling strategy. This approach allows the development of task-invariant risk features that can generalize effectively across different environments.



Concretely, we propose Risk-Informed Policy Learning (RIPL), a framework where a state-centric risk model is used to guide policy learning. RIPL augments the RL agent’s state representation by integrating risk information from the risk model alongside the state description. This framework is formalized as a \emph{Risk-informed MDP}, where the original state is enhanced with risk metrics provided by the risk model. Additionally, we extend this framework to incorporate constraints, thereby adapting it for use with Constrained Markov Decision Processes (CMDPs).  The risk model is trained to estimate the probability that the agent will encounter an "unsafe" state after exactly \( k \) actions, where \( k \in \{ 1, \ldots, H \} \).

RIPL distinguishes itself from existing methods in two key ways. First, traditional approaches for safe or risk-aware exploration often rely on external safety critics—such as filtering or shielding mechanisms—to evaluate and conditionally execute actions. These methods can lead to overly conservative policies that may hinder learning. In contrast, RIPL integrates risk information directly into the policy learning process, allowing for more effective management of high-risk situations. Second, unlike previous risk-aware RL methods that model risk as a scalar value~\citep{intrinsic_fear,csc,sauteRL}, RIPL represents risk as a probability distribution over relative risk values derived from policy rollouts. This probabilistic approach captures more detailed risk information, enabling more nuanced risk-informed decision-making and more accurately approximating important values such as expected returns and constraint violations.






% Concretely, we propose Risk-Informed Policy Learning (RIPL), a framework in which a state-centric risk model is used to inform policy learning. In practice, RIPL is a form of state augmentation in which we condition the RL agent on the output of a risk model in addition to the state description. This notion is formalized as a \emph{Risk-informed MDP} that, given a risk function, augments the original state to include the risk information provided by the risk model. The risk model itself is trained to predict, for a given state, the probability that the agent will encounter an ``unsafe'' state after exactly $k$ actions where $k \in \{ 1, \ldots, H \}$. Though simple, the RIPL framework is distinct from past approaches in two important ways. First, existing approaches for safe or risk-aware exploration largely attempt to reduce the hazards of exploration using safety critics~\citep{learning_to_be_safe,ldm,csc}, where, through mechanisms like filtering or shielding that are external to the policy, actions selected by the policy during exploration are only conditionally executed by the agent pending their evaluation by the safety critic. However, by explicitly restricting the policy from exploring certain states during learning, these approaches often converge to overly conservative solutions, many times preventing learning entirely. Second, unlike previous risk-aware RL methods, RIPL represents risk as a probability distribution over relative risk values learned from data generated by policy rollouts. Modelling risk as a distribution rather than a scalar (e.g. \citep{intrinsic_fear,csc,sauteRL}) captures more nuanced information with which important values such as expected return or expected constraint violations may be bounded or approximated. This representation also naturally allows risk-informed decision-making, rather than simply risk-averse.

% \todo{incorporate below into previous paragraph... near mention of formalizing the risk model}
% Due to its simplicity, RIPL is also broadly applicable. It may be used in both constrained and unconstrained MDPs, uses only the data already available to, or generated by, the RL agent, and requires no additional assumptions or privileged data beyond what is typical in the safe-RL literature. Moreover, RIPL may be used with any underlying RL algorithm allowing essentially all common RL algorithms to be converted to their risk-informed variants.





%Further, training risk-informed agents is very flexible as the risk model may be trained in several ways, including jointly from scratch alongside the policy, pre-trained on a given task and transferred to agents learning new tasks in similar environments, or continually updated over the agent's lifetime. 
%In particular, the risk model may be learned using rollouts from any set of policies. 


Empirically, we investigate two primary hypotheses addressing the key challenges outlined:

\begin{itemize}
    \item Integrating risk information directly into the state representation enhances both the safety and efficiency of reinforcement learning (RL) agents during the learning process.
    \item Since the risk information is learned in a state-centric or policy-agnostic manner, it can be generalized across different tasks, leading to safer and more efficient learning when applied to new tasks.
\end{itemize}


% describe breadth / depth of experiments (domains, etc.)

% highlight outcomes w.r.t. H1-H3

We empirically evaluate risk-informed agents across four distinct simulated robotic environments, encompassing tasks such as manipulation, navigation, and locomotion. Our results demonstrate that risk-informed agents can develop policies that are up to twice as safe during training and up to twice as sample-efficient compared to baseline methods. Additionally, we show that risk information is transferable across different tasks, serving as an effective prior for learning policies in new tasks. We further investigate the risk-reward tradeoff exhibited by risk-informed agents relative to the baselines. We also conduct additional analyses and ablations to validate key design decisions.

% list ablation studies (what knobs did we try turning?)





==> sections/relatedwork.tex <==
\section{Related Work}


Reinforcement learning (RL) agents must efficiently explore the state space to discover optimal policies for specific tasks. Common exploration strategies include stochastic methods like the $\epsilon$-greedy approach, where a random action is chosen with a probability $\epsilon$, and entropy regularization techniques, such as MaxEnt RL, which encourages exploration by maximizing the policy’s entropy~\citep{hao2023exploration,neu2017unified}. Additionally, curiosity-driven approaches provide supplementary rewards for encountering novel situations or reducing model uncertainty~\citep{curiosity_org,rnd,doctor2022learning}. While these methods enhance exploration, they do not explicitly address the challenge of safe exploration, which is essential for deploying RL in real-world applications.

Reinforcement learning (RL) algorithms often need to develop effective policies based on observations of the environment, rather than having direct access to the true state. These observations can come from sensors like RGB cameras, LiDAR, or depth sensors. Learning representations that capture the essential aspects of the environment or task can significantly enhance the performance of RL algorithms. To achieve this, various methods employ auxiliary rewards or alternative training signals \citep{sutton2011horde, jaderberg2016reinforcement,riedmiller2018learning, lin2019adaptive}. One effective approach is learning to predict future states, which has proven valuable in both model-free \citep{munk2016learning,schwarzer2020data,ota2020can} and model-based \citep{watter2015embed,ha2018world} settings in latent space. Additionally, some approaches have explored joint representations for state-action pairs \citep{fujimoto2024sale,liu2021return}.

In this paper, we focus on learning representations that capture safety-related aspects of the environment based on the agent's prior experience. We argue that in most environments, safety or constraints are inherent to the environment or state, rather than the task itself. This means that safety-related information can be learned in a task-agnostic manner, enabling these representations to generalize across different tasks.

The concept of risk has been an object of interest in Markov decision processes since the early 1970s~\citep{howard1972risk}, and specifically in reinforcement learning since the early 2000s (see~\citep{garcia2015comprehensive} for a nice overview). While there are many competing definitions for ``safety'' and ``risk'' within the RL literature~\cite {garcia2015comprehensive}, many find common ground in their focus on the exploration process within RL. 


% There has been considerable research on many sub-problems in RL, including both sample efficiency and safety. Methods for efficient exploration generally fall into one of three categories. Curiosity-driven approaches \cite{curiosity_org, rnd} use a curiosity term in their loss function to encourage exploring novel states; Bayesian \cite{bootDQN, rpf} approaches estimate the posterior distribution of the value function and encourage exploring states with high uncertainty; and distributional RL\cite{dist_rl} approaches reformulate the Bellman update over distributions, allowing algorithms to implicitly model uncertainties in the learning process. While these methods do increase sample efficiency, they make no improvements with respect to safety, and in many cases may be less safe.

% \kaustubh{  
% P3: Safe exploration methods commonly formulate the Rl problem as a constrained MDP. Describe different design choices made by different methods. 
% P4: Our paper is most similar to Conservative Safety Critics, SQRL and Saute RL. What do they do and what do we do differently and why it makes sense. The idea of RIPL can also be compared to methods in Meta-RL that use a context variable to condition policy learning. We are also aiming to learning something that generalizes across tasks (centric to the environment). }


Methods for safe exploration are often formulated as constrained Markov decision processes \citep{cpo,cvpo}. Alternatively, Bayesian model-based methods \citep{thesis_berkenkamp}, represent uncertainty within the model via Gaussian processes, favoring exploration in states with low uncertainty. Other safe exploration methods try to avoid unsafe states by explicitly modeling risk using a safety critic. These so-called filtering or shielding approaches \citep{learning_to_be_safe,ldm,csc} prevent actions during exploration that the critic deems high risk and attempt to guide the agent to remain within the bounds of its experienced data distribution. Due to their cautious approach, these methods are often inefficient and can fail to ensure complete state-space coverage --- a requirement for deriving an optimal policy.

In this paper we relax some of the inherent tradeoffs between sample efficiency and safety by delegating this problem to the agent itself via state-augmentation, allowing the network to figure out how best to use risk information. State-augmentation most often includes either \emph{extra information} or \emph{re-processed information}. Extra information may be added to give the agent access to privileged information as in goal-conditioned RL \citep{liu2022goal}, to retain the Markov property, for example by including action histories when solving MDPs with stochastic delays \citep{nath2021revisiting} or Langrangian weights when solving certain CMDPs as the Lagrangian update is itself Markovian \citep{calvo2023state}. It can also be used in combination with changes to the reward function, such as to reduce the risk of vanilla Q-learning when the objective is sensitive to higher order moments in the distribution of returns \citep{ma2019state}, or in SauteRL \citep{sauteRL}, where states are augmented with the remaining constraint budget and the reward function is modified to reflect safety considerations.

Here, we avoid augmenting our state with extra information as this may not always be available, and instead use re-processing. This strategy has proven effective in meta-RL \cite{bhatia2023rl}, where Q-value augmentation leads to both faster adaptation and better generalization. In the context of safe reinforcement learning, the intrinsic fear approach \cite{intrinsic_fear} trains a model to predict the probability that a given state could reach an unsafe state within $k$ actions. They then modify the agent's loss function by a Lagrange term based on the model output. While this work bounds the sub-optimality of the resulting policy, it assumes optimal policies rarely visit near-failure states, which may in practice be unrealistic (e.g. most robots are often just a few commands from damaging themselves). RIPL is distinct from prior safe exploration methods in several important ways: 1) We do not perturb the original objective; 2) We do not completely prevent exploration of any state; 3) We do not require any domain knowledge; 4) We model risk as a distribution rather than a scalar.


meta-RL relation: risk model is a type of context variable. 


